Approximate Environment Decompositions for Robot Coverage Planning using Submodular Set Cover

In this paper, we investigate the problem of decomposing 2D environments for robot coverage planning. Coverage path planning (CPP) involves computing a cost-minimizing path for a robot equipped with a coverage or sensing tool so that the tool visits all points in the environment. CPP is an NP-Hard problem, so existing approaches simplify the problem by decomposing the environment into the minimum number of sectors. Sectors are sub-regions of the environment that can each be covered using a lawnmower path (i.e., along parallel straight-line paths) oriented at an angle. However, traditional methods either limit the coverage orientations to be axis-parallel (horizontal/vertical) or provide no guarantees on the number of sectors in the decomposition. We introduce an approach to decompose the environment into possibly overlapping rectangular sectors. We provide an approximation guarantee on the number of sectors computed using our approach for a given environment. We do this by leveraging the submodular property of the sector coverage function, which enables us to formulate the decomposition problem as a submodular set cover (SSC) problem with well-known approximation guarantees for the greedy algorithm. Our approach improves upon existing coverage planning methods, as demonstrated through an evaluation using maps of complex real-world environments.

==> Notes/Questions.tex <==
\section{Questions}

\begin{itemize}
    \item Can we use these techniques to come up with our own method that gives us the shapes we want (trapezoids)?
    \item Can we improve/extend these techniques to achieve a decomposition that may give us different shapes, from which we can get trapezoids?
\end{itemize}

==> Notes/StraightSkeleton.tex <==
\section{Using straight-skeleton decomposition}

Investigated using straight skeletons to determine sector orientation.

\begin{itemize}
    \item High-fidelity decomposition - requires a post-processing step still
    \item Identifies coverage orientations for each sub-region.
\end{itemize}

\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{Assets/optimal direction.png}
    \caption{Covering a narrow convex corridor along the boundaries}
    \label{fig:convex-example}
\end{figure}

\begin{figure}[h!]
    \centering
    \subcaptionbox{}{
    \centering
    \includegraphics[width=0.465\linewidth]{Assets/Continuous coverage.png}
    }
    \subcaptionbox{}{
    \centering
    \includegraphics[width=0.465\linewidth]{Assets/Straight-skeleton with offset polygons.png}
    }
    \caption{(a) Covering a general polygon while continuing to follow outer edges. (b) The corresponding straight skeleton of a polygon. Source: Wikipedia}
    \label{fig:shrinking-polygons}
\end{figure}

\begin{figure}[h!]
    \centering
    \subcaptionbox{}{
    \centering
    \includegraphics[width=0.47\linewidth]{Assets/Results/ex1-straight-skeleton.png}}
    \subcaptionbox{}{
    \centering
    \includegraphics[width=0.47\linewidth]{Assets/Results/ex1-sector-decomp.png}
    }
    \caption{(a) Straight skeleton and corresponding faces of a polygon (b) Minimum rotated rectangles of faces to form sectors}
    \label{fig:shrinking-polygons}
\end{figure}

\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{Assets/Results/ex2-sector-decomp.png}
    \caption{For complex environments, minimum rotated rectangles cannot be used. Also, we need a post-processing step to remove overlapping unnecessary sectors}
\end{figure}

\clearpage

\section{October 17-19}

In literature, the edges of the polygon are used as primary evidence to determine coverage orientations \cite{dolgovDetectionPrincipalDirections2009, huangOptimalLinesweepbasedDecompositions2001a}. Consider the simple case of covering a corridor of convex shape (Fig. \ref{fig:convex-example}). The optimal coverage path in this case is trivial: cover along the edges of the corridor regardless of the orientation. In the case of a general polygon, such coverage can still be performed with paths that resemble the shrinking of the outer polygons (Fig. \ref{fig:shrinking-polygons}). We will refer to these shrinking polygons as \textit{offset polygons}. However, the further we move from the boundaries of the polygon, we observe "singularities" in the path: the offset polygon breaks into smaller pieces that are harder to cover (they consist of short line segments that cause the robot to turn during coverage). They can't be ignored either as that may cause gaps in coverage.

An alternate interpretation of such offset polygons however is that it determine a \textit{coverage orientation} for different parts of the environment. Consider a straight skeleton of a polygon as shown in Fig. \ref{fig:shrinking-polygons}(b), and consider partitioning the polygonal environment into sub-regions as determined by the \textit{faces} formed between the skeleton bisectors (blue lines) and the polygonal edges (black lines). Each such sub-region is strongly associated with an edge in the polygon, which provides a coverage orientation for each sub-region. While these orientations are not always optimal if each sub-region is covered individually, the coverage lines obtained using these offset polygons.

\section{October 10-12}

\textbf{Investigated the straight skeleton of a polygon}

\vspace{2mm}

\textbf{Definition:} Consider the continuous shrinking of the edges of a polygon, in which the edges move inwards parallel to themselves at a constant velocity. The straight skeleton of a polygon is defined as the set of curves traced out by the moving vertices in this process.

\vspace{2mm}

For convex polygons, the straight skeleton, the medial axis and the Voronoi diagram are exactly equivalent. For non-convex polygons, they are not necessarily the same as the Voronoi diagram, for the following reasons:
\begin{itemize}
    \item Voronoi boundaries are \textit{equidistant} from both the edges and the vertices of the polygon. The straight skeleton is only dependent on the edges of the polygon.
    \item Voronoi boundaries tend to be \textit{curves}, whereas the straight-skeleton is composed of straight lines as edges.
\end{itemize}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Assets/straight-skeleton vs voronoi.png}
\end{figure}

\vspace{2mm}
\noindent\textbf{Constriction Decomposition Method (CDM)}

\vspace{2mm}

\textit{Authors: Stanley Brown and Steve Waslander}

\vspace{2mm}

Using CGAL to create a \textit{straight skeleton}. CGAL identifies different types of nodes, including \textbf{split} nodes, where the edge of a straight-skeleton at a given point in time during shrinking is split by a reflex vertex in the polygon.

Weighted skeleton - Reason out what we want and if this could work from a principled approach.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Assets/CGAL-output.png}
    \caption{A straight skeleton (red edges) of the polygon with holes (black edges). Green dots signify skeleton nodes, while blue dots signify \textit{split} nodes. The split nodes are used by CDM to decompose the environment.}
\end{figure}

\vspace{2mm}
\textbf{Considerations:}

\vspace{2mm}

Can we allow for overlap?

Can we allow for missed coverage?

==> Old/line_sweep_approach.tex <==
We first identify a set of candidate sectors given an environment, or a subset of the environment. Our sector identification approach is inspired by other environment decomposition approaches such as trapezoidal and boustrophedon decompositions. We employ a line-sweep-based approach where we scan the environment using a sweep line at different orientations to identify parts of the environment that are sweepable.

\begin{figure}
\centering
\includegraphics[width=\linewidth]{Assets/Getting candidate sectors.png}
\caption{The line sweep approach used to obtain the candidate sectors for a single sweep orientation.}
\label{fig:line-sweep}
\end{figure}

\begin{definition}[Reflex vertex]
    Reflex vertex is the vertex of a polygon for which the internal angle formed by the two incident edges is obtuse.
\end{definition}

\textbf{(i) Sweep Orientations:} We first identify all possible coverage path orientations using the environment polygon's edges. To obtain the angles to perform line sweep, we employ a technique called the Probabilistic Hough Transform to extract lines from the given map of the environment. The hough transform obtains lines that depict the orientations of the environment's edges that significantly affect the geometry of the polygon.

\textbf{(ii) Oriented Line Sweep:} For each orientation, we identify sweepable regions in the environment using a line-sweep based approach. This approach is inspired by its usage in computing similar environmental decompositions, such as 

The algorithm is as follows: we sweep a line oriented at each of the identified orientations. Along the line sweep, we identify three different events: (i) \textit{split} events where a segment of the line splits into multiple segments, (ii) \textit{merge} events where line segments merge into a single segment, and (iii) \textit{reflex} events where the line intersects with a reflex vertex of the polygon. Between these events, the sweep lines that are parallel and connected to each other form the sectors for that specific orientation. This is performed for each orientation from step (i).

\textbf{New Sweep line criteria: (i) plane sweep (ii) at each sweep line: is the line split or is it a reflex vertex (iii) get cells at each angle (iv) remove cells where the sweep line endpoints are farther than a certain distance.}

\textbf{(iii) Re-orienting:} Once the sectors are obtained, we check if sweep angle for each sector can be reoriented to improve its coverage. To do this, we compute a rectangular hull of the sector and orient the sweep lines along the longest edge of the rectangle. After re-orientation, we check if any of the reoriented sweep lines are broken by obstacles, in which case, the sector is discarded.

\begin{remark*}[Implementation Note]
    We want sectors that can each be covered by a lawnmower path with little to no coverage overlap. To ensure this requirement is met, we establish an additional criteria that the endpoints of the sweep lines are at-most some $\beta$ times the tool width $l$. While this criteria may increase the number of sectors for each line sweep orientation, we observe that the runtime is not affected by this additional constraint.
\end{remark*}

==> Old/min_set_cover_formulation.tex <==
Our objective is to compute a set of sectors that minimize the cost of the resulting coverage path. Let $J(Q_i)$ be a function that gives the length of the lawnmower path required to cover a sector. Note that a sector is allowed to overlap with obstacles so the lawnmower path may not span the entirety of the sector. The area of the environment $\mathcal{W}$ that can be covered by the coverage path is $|Q_i \cap \mathcal{W}|$, where $\mathcal{W}$ is a constant set. The minimum length of the coverage path for a tool of width $l$ is given by:
\[\frac{|Q_i \cap \mathcal{W}|}{l} \leq J(Q_i).\]
Therefore, one can minimize the length of the coverage path by minimizing the area of $\mathcal{W}$ covered by the sector. Therefore, the objective for the problem is:
\[\min_{Q_i \in \mathcal{Q}} \sum_{i=1}^k |Q_i \cap \mathcal{W}|,\]
where the cardinality operator $|.|$ for a continuous set in $\mathbb{R}^2$ computes the area of the set. We now add a constraint to ensure that the environment is fully covered:
\[\mathcal{W} \subseteq \bigcup_{i=1}^k Q_i.\]

We also add a constraint to ensure that the sectors are large enough to be covered by a coverage tool of width $l$. Consider $w_i$ and $h_i$ to be the width and height of each sector $Q_i$. We enforce that these dimensions be large enough for the area to be covered by the robot as follows:
\[h_i, w_i \geq l.\]

% We also want sectors that fit well into the environment, which is not possible if the sectors are allowed to exceed the environment by a large quantity. To that end, we impose a threshold $\alpha$ on how much of the sector's area can exceed the environment. The following constraint for each sector $Q_i$ captures this requirement:
% \[\frac{|Q_i \setminus \mathcal{W}|}{|Q_i|} \leq \alpha.\]

\begin{problem}[Sector Decomposition]
    Given an environment $\mathcal{W}$, and coverage tool width $l$, compute a set of sectors $\Tilde{Q} = \{Q_1, Q_2, \dots Q_k\}$ that solve the following optimization problem:
    \begin{align}
        \min_{Q_i \in \mathcal{Q}} \quad& \sum_{i=1}^k |Q_i \cap \mathcal{W}|\\
        \text{s.t.} \quad& \bigcup_{i=1}^k Q_i \supseteq \mathcal{W}, \label{eq:environment-contained}\\
        & h_i, w_i \geq l \textrm{ for } 1 \leq i \leq k,
        % & \frac{|Q_i \setminus \mathcal{W}|}{|Q_i|} \leq \alpha.
    \end{align}
    \label{prob:sect_decomp}
\end{problem}

\textbf{Issue with this:}

\begin{itemize}
    \item Some feasible solutions for this formulation are:
    \begin{itemize}
        \item A single rectangle covering everything
        \item A set of small grid cells covering the environment exactly
    \end{itemize}
    both of which we don't want.
\end{itemize}

==> Old/old-sector-decomp.tex <==
%% Problem with some tolerances

% \textit{In a later section, we will remove this assumption and propose algorithms that do not require $\mathcal{Q}$ to be finite.}

% For each sector $Q_i$, we define a clear coverage direction along its \textit{diameter} \textbf{cite Shamos Thesis}. 
% \begin{definition}[Line of support \textbf{cite Shamos}]
%     Given a polygon $P$, a line $L$ is a line of support of $P$ if it meets the boundary of $P$ and $P$ lies entirely on one side of $L$.
% \end{definition}
% \begin{definition}[Diameter of a convex polygon]
%     Given a convex polygon $P$, the diameter length of a convex polygon is the greatest distance between parallel lines of support of $P$.
% \end{definition}
% We will refer to the line segment along which this distance is measured as the diameter line. We look to orient the lawnmower path for each sector along its diameter line to minimize the turns needed to cover the sector. 

We now look to compute $k$ sectors that cover as much of the area $\mathcal{W}$ as possible. Specifically, we look to maximize the following function:
\begin{align*}
    \max_{\Tilde{Q}\subseteq\mathcal{Q}} \quad& |\bigcup \Tilde{Q} \cap \mathcal{W}|,
\end{align*}
where the cardinality operator $|.|$ for a continuous set in $\mathbb{R}^2$ computes the area of the set. To improve the coverage of the decomposition, we consider some tolerances in our sector decomposition for (i) missed coverage ($\alpha$), (ii) overlapping coverage ($\beta$), and (iii) area outside $\mathcal{W}$ ($\gamma$).

We compute missed coverage as the area of $\mathcal{W}$ that is not covered by the union of all sectors. More precisely, we have the following:
\begin{align}
    \alpha = |\mathcal{W} \setminus \bigcup \Tilde{Q}|.
\end{align}
For overlapping coverage, we compute the \textit{total overlapping area} between all sectors by summing the areas of all the sectors and removing the area of the workspace $\mathcal{W}$
\begin{align}
\beta = (\sum_{i \in [1,k]} |Q_i|) - |\bigcup \Tilde{Q}|.
\end{align}
% To ensure that the sectors are covering the workspace, we enforce the following constraint:
% \begin{align}
%     \mathcal{W} \subseteq \bigcup \mathcal{Q}.
% \end{align}
Thirdly, we also allow some tolerance for the sectors to exceed the area of the environment. Specifically:
\begin{align}
    \gamma = |\bigcup \Tilde{Q} \setminus \mathcal{W}|.
\end{align}

% \begin{align}
%     \beta = \max_{i,j \in [1,k], i \neq j} (\text{area}(S_i \cap S_j)).
% \end{align}
Let $\Bar{\alpha}$, $\Bar{\beta}$ and $\Bar{\gamma}$ be maximum thresholds for $\alpha$ and $\beta$ respectively. The objective of the problem now is to compute the minimum number of sectors with these constraints We now pose the main problem we look to solve.

\begin{problem}[Sector Decomposition]
    Given an environment $\mathcal{W}$, an integer $k$, and maximum threshold values $\Bar{\alpha}$, $\Bar{\beta}$, and $\Bar{\gamma}$ for missed coverage, overlapping coverage, and overlap with obstacles respectively, compute a set of sectors $\Tilde{Q} = \{Q_1, Q_2, \dots Q_k\}$ that solve the following optimization problem:
    \begin{align}
        \max_{\Tilde{Q}\subseteq\mathcal{Q}} \quad& |\bigcup_{i=1}^k Q_i \cap \mathcal{W}|\\
        \text{s.t.} \quad& |\Tilde{Q}| \leq k, \label{eq:cardinality-cons}\\
        & |\mathcal{W} \setminus \bigcup \Tilde{Q}| \leq \Bar{\alpha},\\
        & (\sum_{i \in [1,k]} |Q_i|) - |\bigcup \Tilde{Q}| \leq \Bar{\beta},\\
        & |\bigcup \Tilde{Q} \setminus \mathcal{W}| \leq \Bar{\gamma}.
    \end{align}

    \label{prob:sect_decomp}
    
    % \begin{align}
    %     \min_\mathcal{Q} \quad& |\mathcal{Q}|\\
    %     \text{s.t.} \quad& |\mathcal{W} \setminus \bigcup \mathcal{Q}| \leq \Bar{\alpha},\\
    %     & (\sum_{i \in [1,k]} |Q_i|) - |\mathcal{W}| \leq \Bar{\beta},\\
    %     & |\bigcup \mathcal{Q} \setminus \mathcal{W}| \leq \Bar{\gamma}.
    % \end{align}
\end{problem}

\noindent\textbf{NOTES:} 
\begin{itemize}
    \item An alternative config we can consider is to have a $\gamma$ for each sector. This would allow some sectors to be more \textit{precise} and others to be more \textit{encompassing}.
\end{itemize}

==> Old/potato_peeling.tex <==
\section{Potato peeling approach}

The "potato peeling" problem is that of finding the convex polygon of the largest possible area inscribed in a polygonal region $P$ (with or without holes). The potato peeling problem is optimally solvable in $O(n^7)$ time (\textbf{cite Chang and Yap}), where $n$ is the number of vertices of the polygon $P$. However, due to the high order of the polynomial, approximation algorithms for this problem have been developed to improve the runtime with known worst-case performance. The best-known performance guarantee is $(1-\epsilon)$-approximations in near-linear time (\textbf{cite Hall-Holt, Cabello}), where $\epsilon > 0$ is a tolerance to enable the approximation. 

Hall-Holt achieves this approximation factor for computing the largest area triangle/rectangle in polygons with holes in $O(n \log n)$ time. Cabello's algorithm is a randomized algorithm that achieves this guarantee with a probability of at least 2/3 for simple polygons with no holes, albeit while requiring near-linear runtime i.e. an improvement from Hall-Holt.

\vspace{2mm}

Using potato peeling as a greedy step, we propose the following greedy algorithm for sector decomposition:

\textbf{Algorithm:}
\begin{itemize}
    \item Input polygon $P$
    \item Sectors $\Tilde{Q} = \emptyset$ 
    \item While $|\Tilde{Q}| < k$
    \begin{itemize}
        \item $Q \rightarrow$ Largest convex potato in $P$
        \item  $P = P \setminus Q$
        \item $\Tilde{Q} = \Tilde{Q} \cup \{Q\}$
    \end{itemize}
    \item Return $\Tilde{Q}$.
\end{itemize}

\vspace{2mm}

Note that, by solving the potato peeling problem for the greedy step, we remove the assumption that the set $\mathcal{Q}$ is finite. Solving the potato peeling problem optimally after removing the previously computed sector $Q$ maximizes the marginal gain in the area covered. Therefore, no initial set of sectors $\mathcal{Q}$ is required to choose a sector from.

\vspace{2mm}

\noindent\textbf{Guarantee using exact approach:}

\vspace{2mm}

By solving the potato peeling as a greedy step, we can propose a greedy algorithm to solve the sector decomposition problem. The algorithm will then have an approximation factor of $(1 - \frac{1}{e})$, as the greedy step is solved optimally. However, the runtime of the algorithm is $O(kn^7)$, where $k$ is the maximum number of sectors and $n$ is the number of vertices describing the polygonal representation of the set $\mathcal{W}$.

One thing to note however is that the exact approach runs in linear time for polygons with a single reflex vertex (vertex with interior angle $> 180^\circ$). This could potentially lend to parallelization using a GPU, where each reflex vertex is analyzed which could lead to a significant improvement in runtime. 

\vspace{2mm}

\noindent\textbf{Guarantee using approximate approach:}

\vspace{2mm}

Following Downie et. al., the greedy approach using an $\alpha$-approximation algorithm for the potato peeling problem is as follows:
\[f(\Tilde{Q}) \geq (1-e^{-\frac{1}{\alpha}})f(\Tilde{Q}^*),\]
where $\Tilde{Q}^*$ is the optimal solution using the exact approach to the potato peeling problem. Using the $(1-\epsilon)$-approximation algorithm, we have the following approximation guarantee.
\[f(\Tilde{Q}) \geq (1-e^{-\frac{1}{1-\epsilon}})f(\Tilde{Q}^*).\]
This approximation however improves the runtime of the greedy approach to $O(k n \log n)$ for polygons with holes.

\vspace{2mm}

\subsection{Concerns:}
\begin{itemize}
    \item I haven't been able to find a good implementation for any potato peeling algorithms.
    \begin{itemize}
        \item These are complicated algorithms so an implementation for the potato-peeling step may take a bit of time.
        \item \textbf{Update:} Built a prototype with an available implementation for the largest \textit{axis-parallel} rectangle.
    \end{itemize}
    \item The potatoes would not be edge-aligned, meaning that some sub-optimal solutions can be possible.
\end{itemize}

\section{Results}

\subsection{Implementation}

There is no available implementation of the Hall-Holt algorithm. However, we instead used the approach by \textbf{Marzeh et. al.} which computes the largest \textit{axis-parallel} rectangle in a given environment. We then rotated the environment using a step size ($10^\circ$) to compute the largest rectangle in the environment. Once the largest rectangle is computed, we simply remove the area covered by the rectangle from the environment and continue the process. The termination condition is the maximum number of sectors, which in this case is 20.

\newpage

\subsection{Greedy algorithm results}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\linewidth]{Assets/Results/Results - New york - 20 sectors 10 deg diff.png}
    \caption{Greedy sector decomposition results}
    \label{fig:greedy-results-1}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{Assets/Results/Results - 2003 map - 20 sectors 10 deg diff.png}
    \caption{Greedy sector decomposition results - Real-world map \textbf{(Replace with anonymized map later)}}
    \label{fig:greedy-results-2}
\end{figure}


==> Old/prob_def_atom_strip.tex <==
\section{Problem Definition}

Consider a 2D environment represented by the bounded set $\mathcal{W}$. Our goal is to cover this environment with a square tool of width $l$ in the shortest time and length possible. To this end, we consider the coverage of a subset of points $P \subset \mathcal{W}$ such that the coverage of these points results in the coverage of the environment. We consider covering each such point using a set of $\omega$ possible orientations (i.e. 2$\omega$ directions), where each orientation $\phi \in [0^\circ, 180^\circ)$. We model this by considering, for each point $x \in P$, a finite set $O_x$ of infinitely short line segments oriented along each such possible orientation. We call each such line segment an \textit{atomic strip}. The problem we look to solve is the following:

\begin{problem}[Atomic Strip Orienteering]
    Given a subset of points $P$, a finite set $O_x$ of atomic strips to cover a point $x \in P$ along $\omega$ possible orientations, find an atomic strip $o \in O_x$ that constitutes the optimal coverage orientation for $x$.
\end{problem}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Assets/Fekette - Atomic strip cover.png}
    \caption{Example from Fekete et. al. \cite{feketeCoveringToursCycle2019} of using atomic strip covers to plan coverage paths. We intend to solve for the optimal orientations of these strips.}
    \label{fig:atomic_strip_covers}
\end{figure}

The coverage planning problem then is to compute a tour of these oriented atomic strips, which can be formulated as a Generalized traveling salesman Problem (GTSP). However, GTSP is NP-Hard, so we look to minimize the size of the GTSP instance by grouping atomic strips that can be covered sequentially (e.g. along a straight line).

\begin{problem}[Atomic Strip Grouping]
    Given a set of oriented atomic strips that covers all points in $P$, compute an optimal grouping of these strips into path segments that cover the strips in each group sequentially.
\end{problem}

\section{Covering sub-regions}

We have also considered the coverage of entire environments. However, it may be preferential to cover the environment by sub-regions or \textit{sectors}, i.e. covering each sector individually. To this end, we look to group the atomic strips into sectors, by solving the following problem.

\begin{problem}[Sector Decomposition]
    Given a set of oriented atomic strips that covers all points in $P$, compute an optimal grouping of these strips into \textit{sectors} that can be covered individually. The sector decomposition has the following properties:
    \begin{itemize}
        \item Overlap between sectors $\leq o_{\text{max}}$, and
        \item The sectors can miss at-most $p_\text{max}$ points.
    \end{itemize}
\end{problem}

% into a set of $n$ sub-regions, $\{W_1, W_2, \dots W_n\}$ such that, for each $1 \leq i \leq n$ each $W_i \subseteq \mathcal{W}$ and $\cup \{W_1, W_2, \dots W_n\} = \mathcal{W}$.

% Let us consider a function $f$ that takes as input a sub-region $W_i$ and returns a principal axis orientation $\phi_i \in $. Specifically:
% \[f(W_i) = \phi_i.\]

% \vspace{2mm}

% An example of such a function is to take the longest edge in the partition and align the axes parallel and orthogonal to the axis along the edge.

% \vspace{2mm}

% The problem now is to compute a \textbf{partition} of the environment where each partition is covered along its \textbf{principal axes} such that the cost of coverage is minimized.

==> Old/sect-decomp.tex <==
%%% \max_{x \in X, r \in [0,m]} \Bigg\{\frac{\delta_x(S^0)}{\delta_x(S^r)}: \delta_x(S^r) > 0 \Bigg\}

%%% \textit{Runtime:} We now provide a runtime analysis of G-SectD as a function of the input environment's size. Let $v$ be the number of vertices that represent the polygonal region of the environment, including the vertices of the holes in the polygon. 

% \begin{proposition}
%     Given an environment $\mathcal{W}$ with $v$ vertices, each iteration of the G-Sect algorithm has a runtime complexity of $O(v^3 \log v)$.
% \end{proposition}

% \begin{proof}
%     The time required to perform a single line sweep requires $O(v \log v)$ runtime to sort the polygon's vertices and scan the line at each vertex. For $q$ unique orientations, we perform $q$ line sweeps per greedy iteration. However, $q$ is bounded by the number of polygon edges, which is $v$. Therefore, it takes $O(v^2 \log v)$ runtime to compute all sectors.  
    
%     The next source of runtime complexity is the number of comparisons required to make the greedy choice. We assume that the area of each sector can be computed in constant time. The greedy choice runtime is therefore dependent on the number of sectors to compare. For each line sweep orientation, each polygon vertex can border at most 2 sectors. So the number of sectors for each orientation is $O(v)$ and the total number of sectors is $O(v^2)$. The greedy choice can therefore be made in $O(v^2 \log v)$ time, which is the time to sort the sectors based on the area covered. Once the greedy sector is chosen, the polygon difference can be conducted efficiently in $O(v \log v)$ time and does not dominate the runtime complexity.

%     We now analyze how much the size of the polygon changes after each greedy choice. Removing a sector can add at most 2 new vertices, which are the result of the intersection between the sweep line and a polygon edge. However, the resulting vertex is not a reflex vertex and is guaranteed to be included in a subsequently chosen sector. Therefore, this new vertex need not be used for subsequent line-sweeps, which leads to a $O(v)$ polygon for each greedy iteration.

%     Finally, we look at the number of iterations run by G-Sect, given by $m$. Since each line-sweep gives us sector candidates that cover the entire environment, the greedy algorithm must pick a sector decomposition that improves on this. So, the number of sectors is at worst $O(2v)$, as each vertex is at-worst incident with two sectors each. This leads to a total runtime complexity of $O(v^3 \log v)$, proving our proposition.
% \end{proof}



%%% Runtime complexity

    % Number of greedy steps - $O(m)$

    % Complexity of computing polygon difference - $O(n(\mathcal{W}) \log n(\mathcal{W}))$

    % First iteration - $O(n(\mathcal{W})^2 \log n(\mathcal{W}))$

    % Size of the new polygon - 
    % Each vertex in line sweep is in at-most two cells.
    
    % Minimum vertices per cell is 2.

    % Max vertices added by its removal = 2

    % Maximum number of sectors is $O(2 n(\mathcal{W}))$.

    % Number of vertices in the removed polygon $\leq$ n + 2 = O($n(\mathcal{W})$)

    % So total runtime - $O(m n(\mathcal{W})^2 \log n(\mathcal{W})) = O(n(\mathcal{W})^3 \log n(\mathcal{W}))$


% \subsection{Oriented Rank Partitioning}
% Once the sectors are determined, we use this to compute coverage ranks in directions as determined by the sector decomposition. This allows some merges and orientation changes to further optimize the resulting coverage plan. 

% \begin{proposition}[Approximation factor for G-SectD]
%     Let $\mathcal{W}$ be the environment and let $\mathcal{S}^*$ be the optimal solution to Problem \ref{prob:sect_decomp}. Given an $\epsilon$ as the minimum additional coverage ratio, G-SectD computes a solution $\mathcal{S}$ to Problem \ref{prob:sect_decomp} with the following approximation ratio:
%     \[\frac{J(\mathcal{S})}{J(\mathcal{S}^*)} \leq 1 + \ln\frac{1}{\epsilon}\]
% \end{proposition}
% \begin{proof}
% Let $\mathcal{S}^r$ be the sector decomposition obtained after $r$ iterations of the greedy algorithm. We know that at step $0$, $\mathcal{S}^0 = \emptyset$. Also, recall that $\delta_{Q}(\mathcal{S})$ is the marginal return obtained from the addition of sector $Q$ to $\mathcal{S}$. From Theorem \ref{thm:wolsley}, we have the following approximation ratio for the greedy algorithm:
% \[\frac{J(\mathcal{S})}{J(\mathcal{S}^*)} \leq 1 + \ln\bigg( \max_{Q \in \mathcal{Q}, r \in [0,m]} \Bigg\{\frac{\delta_x(\emptyset)}{\delta_x(S^r)}, \delta_x(S^r) > 0 \Bigg\} \bigg).\]

% Note that we eliminate all sectors where $\delta_{Q}(\mathcal{S}) < \epsilon |\mathcal{W}|$, so $\delta_{Q}(\mathcal{S}^r)$ is never 0. Therefore, we look to compute an upper bound for the ratio of marginal returns to obtain a bound for the greedy algorithm. Note that since there may be environment where a single sector may cover the whole environment (e.g. a rectangular environment), we have the following bound for $\delta_x(\emptyset)$:
% \[\delta_x(\emptyset) \leq |\mathcal{W}|.\]
% Therefore, we can obtain the following bound for the ratio of marginal returns:
% \begin{align*}
%     \frac{\delta_x(\emptyset)}{\delta_x(S^r)} \leq \frac{|\mathcal{W}|}{\epsilon |\mathcal{W}|} = \frac{1}{\epsilon}.
% \end{align*}
% This bound proves our proposition as the maximum value of the ratio never exceeds this upper bound.
% \end{proof}
% \begin{remark*}
%     Note that setting $\epsilon = 1$ achieves an approximation factor of 1, indicating that the greedy algorithm obtains the optimal solution. However, this eliminates any sector that does not cover the entire environment, meaning that the only case where this works is when the entire environment is sweepable (e.g. simple convex polygons). For more realistic environments, $\epsilon$ represents a tradeoff to consider between the optimality of the decomposition and the area covered.
% \end{remark*}


% \textit{A more detailed proof:}
    % Let us assume that the property of diminishing returns does not hold for this. As a result, we have the following:
    % \begin{align}
    % &|\bigcup (A \cup \{q\}) \cap \mathcal{W}| - |\bigcup A \cap \mathcal{W}| < |\bigcup (B \cup \{q\}) \cap \mathcal{W}| - |\bigcup B \cap \mathcal{W}|.
    % \end{align}
    % Now, we look to deconstruct the terms on either side of the inequality by exploiting the following property of the area of a set:
    % \begin{align}
    %     |A \cup B| = |A| + |B| - |A \cap B|.
    % \end{align}
    % Using this, we can rewrite the LHS of the inequality as follows:
    % \begin{align*}
    %     |\bigcup (A \cup \{q\}) \cap \mathcal{W}| - |\bigcup A \cap \mathcal{W}| &= |(\bigcup A \cup \bigcup\{q\}) \cap \mathcal{W}| - |\bigcup A \cap \mathcal{W}|,\\
    %     &= |(\bigcup A \cap \mathcal{W}) \cup (\bigcup\{q\} \cap \mathcal{W})| - |\bigcup A \cap \mathcal{W}|,\\
    %     &= |(\bigcup A \cap \mathcal{W}) \cup (q \cap \mathcal{W})| - |\bigcup A \cap \mathcal{W}|,\\
    %     &= |\bigcup A \cap \mathcal{W}| + |q \cap \mathcal{W}| - |(\bigcup A \cap q) \cap \mathcal{W}| - |\bigcup A \cap \mathcal{W}|,\\
    %     &= |q \cap \mathcal{W}| - |(\bigcup A \cap q) \cap \mathcal{W}|
    % \end{align*}
    % Subbing this back in the inequality, we have the following:
    % \begin{align*}
    %     |q \cap \mathcal{W}| - |(\bigcup A \cap q) \cap \mathcal{W}| &< |q \cap \mathcal{W}| - |(\bigcup B \cap q) \cap \mathcal{W}|,\\
    %     |(\bigcup B \cap q) \cap \mathcal{W}| &< |(\bigcup A \cap q) \cap \mathcal{W}|,
    % \end{align*}
    % which contradicts the overlap property as determined above. Therefore, by contradiction, the property of diminishing returns applies for this case, thereby proving the proposition.

==> Sections/Related_works.tex <==
\section{Related Works}

Decomposing an environment to generate a coverage path is not a new concept. It is a vital part of exact decomposition methods, which decompose the environment into cells that can each be covered individually. Boustrophedon Cell Decomposition (BCD) is a popular method that computes a cell decomposition and covers each cell using a lawnmower path \textbf{cite}. Later improvements of BCD optimized this by covering the cells along their optimal directions (that minimize turns). Huang proposed a line-sweep-based method to decompose the environment into convex cells. Specifically, a number of line-sweeps at different angles were conducted to decompose an environment into cells that minimize the sum of \textit{altitudes} of all the cells. However, Huang's approach has an exponential complexity in the worst-case. Other approaches (\textbf{cite Agarwal, Bahnemann}) propose simplified versions of Huang's algorithm to improve runtime complexity at the cost of any optimality guarantees, by picking only one line-sweep angle to decompose the environment.

Outside of coverage planning literature, area decompositions are used to plan obstacle-avoiding robot paths:
\begin{itemize}
    \item Planning algs book: Trapezoidal and other decomps to get roadmaps
    \item Deits and Tedrake: Computing large convex regions
    \item Werner et. al. : Approximating Robot Configuration Spaces with few Convex Sets using Clique Covers of Visibility Graphs
\end{itemize}

"Potato peeling" problem: finding the largest convex set inscribed within a polygon.
\begin{itemize}
    \item Chang et. al: Polynomial solution for potato-peeling problem (O($n^7$) time complexity, O($n^5$) space complexity, simple polygon)
    \item Keikha: Linear-time alg for largest inscribed polygon (disadvantage: convex polygons only)
    \item Hall-Holt et. al.: Finding large sticks and potatoes in polygons (O(n log n) algorithm to find the maximum-area inscribed triangle with approx factor O(1) (i.e. constant)).
    \begin{itemize}
        \item Also, some guarantees on maximum-area ellipses.
    \end{itemize}
    \item Choi et. al.: Maximum area and Maximum perimeter rectangles in polygons.
\end{itemize}

==> Sections/trash.tex <==
% The first problem is that we look to identify a set of candidate sectors $\mathcal{Q}$ for the environment, where each sector can be covered individually by a continuous lawnmower path.

% \begin{problem}[Sector Identification]
%     Given an environment $\mathcal{W}$, compute a set of candidate sectors $\mathcal{Q} = \{Q_1, Q_2, \dots Q_n\}$, where each $Q_i$ represents an area of the environment that can be covered by a continuous lawnmower path.
%     \label{prob:sect_id}
% \end{problem} 

% For each sector $Q_i$ and orientation $\theta_i$, let $J(Q_i, \theta_i)$ be the cost of covering the sector along $\theta_i$. Our objective is to determine a subset $\mathcal{S} \subseteq \mathcal{Q}$ of sectors that minimize the total cost as follows:
% \[\min_{\mathcal{S} \subseteq \mathcal{Q}} \sum_{Q_i \in \mathcal{S}} J(Q_i, \theta_i).\]

% Another goal of the decomposition is to ensure that the entire environment is covered by the subset $\mathcal{S}$. For this, we consider a measure of the area covered by the sectors. 

% We also add a constraint to ensure that the sectors considered are large enough to be covered by a coverage tool of width $l$. Consider $w_i$ and $h_i$ to be the width and height of each sector $Q_i$. We enforce that these dimensions be large enough for the area to be covered by the robot as follows:
% \[h_i, w_i \geq l.\]


%% TRASH CAN

% Let $\alpha$ represent the area of  Therefore, we enforce the following constraint 

% Given this definition, we look to compute a subset $\mathcal{Q}' \subset \mathcal{Q}$ that maximize the coverage of the environment $\mathcal{W}$ using these sectors:

% \[\max_{\mathcal{Q}' \subseteq \mathcal{Q}} |\bigcup_{Q_i \in \mathcal{Q}'} Q_i|.\]

% Now, let us consider the coverage of the environment resulting from covering each sector individually. 

% \[\sum_{Q_i \in \mathcal{Q}'} \min_{\theta_i \in [0, \pi)} J(Q_i, \theta_i) \leq B.\]



% Note that the sectors are free to assume any orientation.

% We also restrict sectors such that there are no collinear coverage lines in the path covering a sector, i.e. no "split" coverage path. Therefore, the robot only takes $90^\circ$ turns at the end of each coverage line. However, note that the sectors are free to assume any orientation.

% \subsection{Sector Grouping}

% Given a sector decomposition of the environment $\mathcal{W}$, we now look to group the sectors into clusters that each correspond to a coverage \textit{assignment}, i.e. covered in a single run. 

% \begin{problem}[Sector Grouping]
%    Given a decomposition of an environment $\mathcal{W}$ into sectors $\mathcal{S} = \{S_1, S_2, \dots, S_k\}$, compute a grouping $\{\mathcal{G}_1, \dots, \mathcal{G}_p\}$ of the sectors into clusters, where each $\mathcal{G}_i \subseteq \mathcal{S}$ for all $i \in [1,p]$, such that each cluster is coverable in a single run.
% \end{problem}





% and consider adding a new sector $q \in \mathcal{Q} \setminus B$. Note that even though $q \notin B$, the area of $\mathcal{W}$ covered by $q$ may already be covered entirely by $A$ or $B$. WLOG, we assume that $q \cap \mathcal{W} \not= \emptyset$. We now verify whether the above inequality holds for the following cases:
    % \begin{itemize}
    %     \item \textbf{Case 1:} $q \subseteq \bigcup A$,
    %     \item \textbf{Case 2:} $q \subseteq \bigcup B$ and $q \not\subseteq \bigcup A$,
    %     \item \textbf{Case 3:} $q \not\subseteq \bigcup B$.
    % \end{itemize}
    
    % \noindent\textbf{Case 1:} If $q \subseteq \bigcup A$, then we have:
    %  \begin{align}
    % &a(\bigcup (A \cup \{q\})) - a(\bigcup A) = 0,\\
    % &a(\bigcup (B \cup \{q\})) - a(\bigcup B) = 0.
    % \end{align}
    % Therefore, the property of diminishing returns holds trivially for this case.

    % \vspace{2mm}
    
    % \noindent\textbf{Case 2:} If $q \subseteq \bigcup B$ and $q \cap \mathcal{W} \not\subseteq \bigcup A \cap \mathcal{W}$, then we have:
    %  \begin{align}
    % &a(\bigcup (A \cup \{q\})) - a(\bigcup A) > 0,\\
    % &a(\bigcup (B \cup \{q\})) - a(\bigcup B) = 0.
    % \end{align}
    % Again, the property of diminishing returns holds trivially for this case.
    
    % \vspace{2mm}
    
    % \noindent\textbf{Case 3:} If $q \cap \mathcal{W} \not\subseteq \bigcup B \cap \mathcal{W}$, following $A \subseteq B$, it must hold that: 
    % \[a(\bigcup B \cap (q \cap \mathcal{W})) \geq a(\bigcup A \cap (q \cap \mathcal{W})).\] 
    
    % In other words, the area of $\mathcal{W}$ covered by $q$ has a larger overlap with the area covered by set $B$ than that of set $A$. Due to the smaller overlap with $A$, the marginal return of adding the sector $q$ to set $A$ must be larger than adding it to set $B$. Therefore, the property of diminishing returns holds for this case as well, proving our lemma.



% We first obtain a set of candidate sectors by computing regions in the environment that can be swept by the robot along an unbroken path. This requirement helps identify sections of the environment that must be covered along the same coverage orientation. We first establish the criteria for a polygon to be sweepable, and propose an algorithm to obtain the candidate sectors.


% Let $Q_i$ be a sector, and let ${l}$ be the set of sweep lines used to cover $Q_i$. We deem $Q_i$ to be sweepable if it satisfies the following criteria:
% \begin{enumerate}
%     \item \textit{Sweep line non-collinearity}: No two sweep lines in the sector can be collinear.
%     \item \textit{Pairwise length variation:} Sweep lines must have a length difference of less than $\alpha$ with its neighboring lines.
%     \item \textit{Pairwise midpoint distance:} The midpoint of a sweep line must be within $\beta$ distance away from its neighbors.
% \end{enumerate}
